Link Prediction via Higher-Order Motif Features

Link prediction requires predicting which new links are likely to appear in a graph. Being able to predict unseen links with good accuracy has important applications in several domains such as social media, security, transportation, and recommendation systems. A common approach is to use features based on the common neighbors of an unconnected pair of nodes to predict whether the pair will form a link in the future. In this paper, we present an approach for link prediction that relies on higher-order analysis of the graph topology, well beyond common neighbors. We treat the link prediction problem as a supervised classification problem, and we propose a set of features that depend on the patterns or motifs that a pair of nodes occurs in. By using motifs of sizes 3, 4, and 5, our approach captures a high level of detail about the graph topology within the neighborhood of the pair of nodes, which leads to a higher classification accuracy. In addition to proposing the use of motif-based features, we also propose two optimizations related to constructing the classification dataset from the graph. First, to ensure that positive and negative examples are treated equally when extracting features, we propose adding the negative examples to the graph as an alternative to the common approach of removing the positive ones. Second, we show that it is important to control for the shortest-path distance when sampling pairs of nodes to form negative examples, since the difficulty of prediction varies with the shortest-path distance. We experimentally demonstrate that using off-the-shelf classifiers with a well constructed classification dataset results in up to 10 percentage points increase in accuracy over prior topology-based and feature learning methods.

==> exp-final.tex <==
% !TEX root =  vldb_main.tex
\section{Experiments \& Evaluation}
\label{sec:exp}
This section describes how we apply and evaluate the motif features for classification to three different graphs.
In particular, we look at the predictive power of motif features for different motif sizes.
We compare different methodologies for feature extraction.

%In this paper, we apply our classification model in three different graphs to reflect  different link prediction applications. 
%In Section \ref{dataset}, we present detailed description of these  datasets.  Experiments settings, implementation details,  tools and platform used are described in Section \ref{Setup}. We demonstrate the accuracy of classification using the two different  approaches for creating training and testing datasets in Section \ref{results}. In Sections \ref{ttest} , \ref{dest} and \ref{Negative} , we present a set of sensitivity analysis to measure the robustness of the classification.


\subsection{Datasets}
\label{sec:dataset}
We use three real-world graphs coming from different domains: Amazon, CondMat, and AstroPh.
The three datasets are from the Koblenz Network Collection. \footnote{\url{http://konect.uni-koblenz.de}}
Table~\ref{tab:dataset} shows more detailed informations and statistics about them.

The first graph represents the co-purchase network of products of Amazon.
It is the graph upon which the ``customers who bought that also bought this'' feature is built.
The nodes are products, and an edge between any two nodes shows that the two products have been frequently bought together.
In this application domain, link prediction tries to model the creation of an association between two products.
In other words, it can help identify hidden relationships between products, which can then be used in a customer-facing recommendation system.

The second dataset, CondMat, is a bipartite graph which represents a subset of authorship relations between authors and publications in the arXiv condensed matter physics section.
Nodes are authors (first set) or papers (second set).
An edge represents that an author has written a given paper.
Link prediction can identify whether an author is a likely contributor of a research paper, for instance, to identify missing records.

The third and final dataset, AstroPh, is a collaboration graph.
In particular, it contains data about scientific collaboration between authors in arXiv's Astrophysics section.
Each node in the graph represents an author of a paper, and an edge between two authors represents a common publication.
Predicting future collaborations between authors based on their previous publications is a well-known application for link prediction. 

\begin{table}[b]
  \centering
  \caption{Basic statistics about the graph datasets.}
  \label{tab:dataset}
  \begin{tabular}{lrrrrrr}
	\toprule
	\textbf{Graph} & \boldmath $\lvert \textbf{V} \rvert$ & \boldmath $\lvert \textbf{E} \rvert$ & \textbf{Avg. degree} & \textbf{Diameter} \\
	\midrule
	Amazon	& \num{334863}	& \num{925872}	& \num{5.5299}		& 47 \\
	CondMat	& \num{22015}		& \num{58595}		& \num{3.0250}		& 36 \\
	AstroPh		& \num{18771}		& \num{198050}	& \num{21.1020}	& 14 \\
	\bottomrule
\end{tabular}
\end{table}

\iffalse
\begin{table}
  \centering
  \caption{More statistics about the graph datasets.}
  \label{tab:dataset2}
  \begin{tabular}{lrrrrrrr}
	\toprule
	\textbf{Graph} &  \textbf{Directed?}   & \boldmath $\lvert \textbf{V} \rvert$ & \boldmath $\lvert \textbf{E} \rvert$  & \textbf{Avg. degree} & \textbf{Diameter}  & \textbf{bipartite?} &  \textbf{Vertex} \\
	\midrule
	Amazon	& No &  \num{334863}	& \num{925872}		&  \num{5.5299}		& 47  & No & product \\
	CondMat	& No	& \num{23133} & \num {93497} 	& \num{3.0250}		& 14 & No  & Author \\
	AstroPh		& No	& \num{18771}		& \num{198050} & \num{21.1020}	& 14  & No & Author \\
	\bottomrule
\end{tabular}
\end{table}

\fi

\subsection{Experimental Settings}
For each graph, we extract a classification dataset for which we compute node pair features.
We extract a uniform sample of edges from each graph as positive examples.
For negative examples, we extract pairs of nodes from the graph which are at distance $2$ or $3$ hops.
Table~\ref{tab:sample} shows the number of examples chosen from each graph.
As already mentioned, to assess the predictive power of the motif features in a simple setting, we build balanced classification datasets.

For each example edge in the datasets, we extract the motifs it occurs in by using a parallel graph mining framework~\cite{teixeira2015arabesque}.
We then group by motif, count the occurrences, and finally normalize the counts to create a feature vector for each example edge which represents the motif distribution of the neighborhood of the edge.

To train the classification models we use the scikit-learn Python library~\cite{scikit-learn}.
All the classification performance results are computed via 10-fold cross-validation.

\spara{Baselines.}
We use several baselines, which we divide in two types.
The first type represents traditional topological features based on triangle closure.
These features include common neighbors (CN), Jaccard coefficient (JC), Adamic/Adar measure (AA), and Preferential Attachment (PA).
The second type is matrix decomposition, which is a commonly used link prediction algorithm.
For these features we use the scores obtained from a non-negative matrix factorization (NMF) trained on the graph with positive edges removed.
This methodology follows the common approach used in the literature.
We use the NMF algorithm available in scikit-learn, and use $100$ factors for the decomposition.

%For each set of edges, we extract motifs that formulated from different number of nodes.
%We use Arabesque Graph platform to extract the motif for the set of sampled edges.
%Then we develop a code to extract the features from motif shapes.
%For each shape we look into edges that comprised it and part of our sample.
%We count the number of times the edge appears in each motif shape extracted from the whole graph.
%We use the counts of each shape as a separated feature.
%We train different set of classifiers for each set of features formulated from the same size of shape. 
%We use Sklearn machine learning platform for training and testing different classifiers.

\begin{table}[t]
	\caption{Number of positive and negative edges sampled for the classification task for each graph.}
	\label{tab:sample}
	\begin{center}
	\begin{tabular}{lrr}
	\toprule
	\textbf{Graph} & \textbf{\# Positive Edges} & \textbf{\# Negative Edges}  \\
	\midrule
	Amazon	& \num{20000}	& \num{20000} \\
	CondMat	& \num{2000}	& \num{2000}   \\
	AstroPh 	& \num{5000}	& \num{5000}   \\
	\bottomrule	
	\end{tabular}
	\end{center}
\end{table}


\subsection{Evaluation Metrics}
We evaluate the classification task via the following three metrics:
\begin{squishlist}
\item Accuracy: the fraction examples correctly classified (true positives and true negatives) over the total number of examples (N).
\[
\frac{TP+TN}{N}.
\]
Given that the classification datasets are balanced, accuracy is a reasonable measure of performance.

\item  Area Under the Curve (AUC): the area under the ROC curve generated from the scores produced by the classifiers.

\item False Positive Rate: the ratio between the number of negative edges wrongly classified (false positives) and the total number of negative edges in the dataset.
\[
 \frac{FP}{FP+TN}.
\]
This measure is useful to understand the effect of graph distance of the negative examples on the classification task.

\end{squishlist}

%We applied the classification using  features computed  by two different extraction methods. The classification accuracy was different between different graph datasets, which require a statistical measurement  to compare between different results.
%
%The most straightforward way to compare classifiers is to compute the average over  different settings for same data sets;
% which is to statistically verify the hypothesis of improved performance by one method among other. by assessing statistical significance of differences.
%In our method, we  obtained the accuracy  from repeated stratified random splits onto training and testing data sets using typical from cross-validation method.
% 
% A common way to test whether the difference between two classifiers’ results over various data sets is non-random is to compute a paired t-test, which checks whether the average difference in their performance over the data sets is significantly different from zero. Thus, we can over justify one method among other.
% 
% 
%We performed the classification  for link prediction on the three dataset using two proposed methods for feature extraction (Remove Real Edges from the graph or Insert Fake Edges into the graph). For each dataset, we analysis the performance of the prediction.
%\textbf{Prediction Accuracy} We now demonstrate the performance results for the our methods in Table 1. It can be seen that our proposed prediction method outperforms the other two comparison methods.


\begin{table}[htpb]
  \caption{Classification performance on Amazon (\rmve).}
  \centering
  \label{tab:ACC-amz-rmv}
  \begin{tabular}{llrrrr}
\toprule
     Metric & Classifier& \multicolumn{4}{c}{Features} \\
	\cmidrule(lr){3-6}
      &  & 3-Motif  & 4-Motif &  5-Motif & Combined  \\ 
\midrule
\multirow{6}{*}{Acc. (\%)} 
	& NB		& \num{57.6} & \num{52.4} & \num{52.7} & \num{52.0} \\
	& LR		& \num{56.5} & \num{59.4} & \num{68.0} & \num{64.4} \\
	& DT		& \num{57.6} & \num{69.4} & \num{70.8} & \num{70.6} \\
	& KNN	& \num{51.5} & \num{69.9} & \num{71.4} & \num{71.0} \\
	& GB	& \num{58.0} & \num{73.3} & \num{76.6} & \num{76.9} \\
	& RF		& \num{57.6} & \num{71.6} & \num{76.3} & \num{77.0} \\
\midrule
\multirow{2}{*}{AUC}
	& GB	& \num{0.58} & \num{0.72} & \num{0.76} & \num{0.76} \\
	& RF		& \num{0.58} & \num{0.72} & \num{0.76} & \num{0.77} \\
\midrule	
\multirow{2}{*}{FPR}
	& GB	& \num{0.11} & \num{0.30} & \num{0.26} & \num{0.27} \\
	& RF		& \num{0.11} & \num{0.32} & \num{0.27} & \num{0.27} \\
\bottomrule

\end{tabular}
\end{table}

\begin{table}[htpb]
\centering
  \caption{Classification performance on Amazon (\inse).}
  \label{tab:ACC-amz-ins}
  \begin{tabular}{llrrrr}
\toprule
     Metric & Classifier& \multicolumn{4}{c}{Features} \\
	\cmidrule(lr){3-6}
      &  & 3-Motif  & 4-Motif &  5-Motif & Combined  \\ 
\midrule
\multirow{6}{*}{Acc. (\%)}
	& NB		& \num{57.7} & \num{57.2} & \num{52.7} & \num{53.6} \\  
	& LR		& \num{62.5} & \num{67.7} & \num{70.0} & \num{67.5} \\    
	& DT		& \num{67.9} & \num{66.9} & \num{69.6} & \num{71.0} \\ 
	& KNN	& \num{63.6} & \num{66.0} & \num{64.0} & \num{65.0} \\  
	& GB	& \num{68.2} & \num{75.0} & \num{76.6} & \num{79.4} \\
	& RF		& \num{68.0} & \num{74.8} & \num{77.0} & \num{79.6} \\ 
\midrule
\multirow{2}{*}{AUC}
	& GB	& \num{0.69} & \num{0.74} & \num{0.76} & \num{0.80} \\ 
	& RF		& \num{0.68} & \num{0.75} & \num{0.78} & \num{0.80} \\
\midrule
\multirow{2}{*}{FPR}
	& GB	& \num{0.25} & \num{0.25} & \num{0.25} & \num{0.18} \\ 
	& RF		& \num{0.23} & \num{0.23} & \num{0.21} & \num{0.18} \\ 
\bottomrule
\end{tabular}
\end{table}

%%% RMV vs INS
\subsection{Removing Positive Edges vs Inserting Negative Edges}
Tables~\ref{tab:ACC-amz-rmv} and~\ref{tab:ACC-amz-ins} show the classification results of the two feature extraction methods (\rmve and \inse, respectively) on the Amazon dataset (the largest one).
We report the accuracy for all the combinations of classifier and motif features.
Combined refers to using all three sets of features (for $k=3,4,5$) as a single feature vector.

By looking at the difference between the tables, it is clear that \inse consistently produces better results than \rmve.
The difference grows smaller as we add more complex features, however for the two best classifiers (GB and RF) \rmve is still $\approx 3\%$ better.
The simpler classifiers do not seem able to exploit the full predictive power of the motif features.
We report more detailed performance numbers for the two best classifiers.
The AUC and FPR are very similar, and the two classifiers are almost undistinguishable.
As expected, the more complex motif features (i.e., larger $k$) work better, and the combination of all three sets is usually the best.
For ease of presentation, henceforth we report results only by using the RF classifier, but we obtain similar results with GB.

Figure~\ref{fig:accuracy} reports the accuracy numbers for RF on all three datasets, for both feature extraction methods.
The results are consistent with what observed above: \inse is consistently better than \rmve.
Interestingly, \inse with just 3-motif features perform better than \rmve with Combined motif features on the CondMat and AstroPh datasets.

We perform a statistical test to compare the classification accuracy of the two methods, \inse and  \rmve.
We obtain $100$ different accuracy results by training the RF with different seeds for the PRNG.
We use Student's t-test to compare the results, and we are able to reject the null hypothesis that the two methods have the same average performance at the $p = 0.05$ significance level.
We conclude that the accuracy of the RF with \inse feature extraction is better than the one with \rmve, and the difference is significant.
It is clear that the \inse feature extraction method is superior, and we return to the reason behind it in Section~
\ref{sec:distribution}.


More complex motif features perform better, with the combination of all of them edging out on the single features.
The latter result might seem surprising, as one would expect the 5-motif features to supersede the smaller ones.
Nevertheless, consider that our 5-motif features do not encode positional information, i.e., we do not know in which part of the 5-motif the edge appears.
Smaller features can supplement this information.
For example, if an edge presents feature m5.3, it could be any of its edges.
But if it also presents no instances of feature m3.2, then we can pinpoint it to be the only edge not involved in any triangle, i.e, the bottom right edge.

Finally, Table~\ref{tab:class-perf} reports Accuracy, AUC, and FPR for RF on all datasets for the two different extraction methods when using the Combined features.
The combination of RF, Combined motif features, and \inse feature extraction is the one that performs consistently on top.
Therefore, we use it when comparing our proposal with baseline methods.


\begin{figure}
\centering
\subfloat[Amazon]
{\includegraphics[width=0.8\columnwidth]{images/AmazonAccuracy.pdf}}  \\
\subfloat[CondMat]
{\includegraphics[width=0.8\columnwidth]{images/comAccuracy.pdf}} \\
\subfloat[AstroPh]
{\includegraphics[width=0.8\columnwidth]{images/arvixAccuracy.pdf}} \\
\caption{Classification accuracy of Random Forest (RF) when using different motif features and different feature extraction methods (\rmve vs \inse).} 
\label{fig:accuracy} 
\end{figure} 

\begin{table}[tbp]
  \caption{Classification performance of Random Forest (RF) with combined motif features when using different feature extraction methods (\rmve vs \inse).}
  \label{tab:class-perf}
  \centering
  \begin{tabular}{llrrr}
\toprule
    \textbf{Method} & \textbf{Graph} & \textbf{Accuracy (\%)}  & \textbf{AUC} & \textbf {FPR} \\
\midrule
\multirow{3}{*}{\rmve}
	& Amazon		& \num{77.0} & \num{0.77} & \num{0.27} \\
	& CondMat	& \num{79.0} & \num{0.79} & \num{0.04} \\
	& AstroPh		& \num{84.0} & \num{0.84} & \num{0.30} \\ 
\midrule
\multirow{3}{*}{\inse} 
	& Amazon		& \num{79.6} & \num{0.80} & \num{0.18} \\
	& CondMat	& \num{96.0} & \num{0.96} & \num{0.04} \\
	& AstroPh		& \num{96.5} & \num{0.97} & \num{0.02} \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[tbp]
  \centering
  \caption{ Prediction Accuracy using neural network framework}
  
  \label{tab:nurual}
  \begin{tabular}{l r r r r}
   \toprule
   \textbf{dataset} &	\textbf{Train Edges} &	\textbf{Test Edges} &	\hspace{1em}\textbf{Accuracy}  & \hspace{1em}\textbf{AUC} \\ 
      \midrule 
  Amazon	&  16000 &   4000 & 99  &  97. 8\\ %   acc 0.99950 auc 0.87419 /  acc 0.99950 auc 0.97856
  CondMat &  4000 & 1000 &  99.3 & 97\\ %93.3 \\ %
  AstroPh &  1600  &  400 &   99.5 & 96.7\\ %91.6  \\ %  average test of epoch 49: loss 0.02657 acc 0.99502 auc 0.96750
   \bottomrule
   
      \midrule 
 % Amazon	&  16000 &   4000 & 86.5  \\
  %CondMat &  4000 & 1000 & 89.3 \\
  %AstroPh &  1600  &  400 &  87.1  \\
   \bottomrule
\end{tabular}
\end{table}






%%%%%%different B values and katz
%% katz= (number of paths) * B+ .., matrix multiplication 
%%%%%%modified comparison table
\begin{table*}[tbp]
  \centering
  \caption{New values Accuracy of the RF classifier (\%) when insert fake edges (\inse) vs baseline features (topological and NMF).}
 
  \label{tab:comparison4}
  \begin{tabular}{l r r r}
   \toprule
   \textbf{Feature} &	\textbf{Amazon} &	\textbf{CondMat} &	\hspace{1em}\textbf{AstroPh} \\
   \midrule
   Jaccard Coefficient	&     61.7 		&	81.1	 &   85.2 \\
   Adamic/Adar	 				& 61.5 		&	74.7    	 &			 75 \\
   Preferential Attachment  & 		 55.0   	& 	61. 2   	&  64.2 \\
   Common Neighbors					  & 64.6       &   78.6  	&  81.2 \\
   Rooted Page Rank 					& 53.2    &   62 &               65 \\ 
   katz , B =0.5 							&    72.5   		&    86  		&  60.2 \\
   katz , B =0.25 							& 72.7		&  	86  		& 	58.2  \\
   katz ,  B = 0.1 	            				& 72.5 		  &   87  	& 	 50 \\
   katz , B= 0.05 	           				&  72   	&   85    	&  50  \\
   Topological combined  ALL 		&  74.8      		& 	86.9   	& 		92 \\
   Topological combined (No PR)  &    74.2 	&   	85.2      &    89.1 \\ 
   Topological combined (No katz)  	&  68 & 	86 .4        &    89.6  \\ 
   
   katz- matrix , B =0.5 							&   52.0 		&       56  				&   60\\
   katz- matrix , B =0.25 							& 53.0 				&   	56				&  00 \\
   katz- matrix ,  B = 0.1 	            				& 60			    &      55  					& 	 59 \\
   katz- matrix , B= 0.05 	           				& 68     			&      52.5      		 		&  00  \\   
   Topological combined (No pageRank)  & 69 & 	85.2            &    00   \\ 
    Topological combined  		&  73      		& 	86.9   					& 		87  \\
   
   \midrule
   NMF																					& 52.0    & 54.0 &                53.5 \\
   NMF + Topological combined											&  73		&  85.9           &    89  \\
   \midrule
   Motif Combined							 									& 79.6     & 96.0        &   96.5 \\
   \bottomrule
\end{tabular}
\end{table*}

%%%%%%different B values and katz
%% katz= (number of paths) * B+ ..
%%%%%%modified comparison table
\begin{table*}[tbp]
  \centering
  \caption{New values Accuracy of the RF classifier (\%) when using combined Motif features (\inse) vs baseline features (topological and NMF).}
 
  \label{tab:comparison3}
  \begin{tabular}{l r r r}
   \toprule
   \textbf{Feature} &	\textbf{Amazon} &	\textbf{CondMat} &	\hspace{1em}\textbf{AstroPh} \\
   \midrule
   Jaccard Coefficient	&     61.7 		&	81.1	 &   85.2 \\
   Adamic/Adar	 				& 61.5 		&	74.7    	 &			 75 \\
   Preferential Attachment  & 		 55.0   	& 	61. 2   	& 64.2 \\
   Common Neighbors					  & 64.6       &   78.6  	& 81.2 \\
   Rooted Page Rank 					& 66.9    &  64.2   & 63.7\\ 
   katz , B =0.5 							&    66.3   		&    73  		&  60.2 \\
   katz , B =0.25 							& 66.1 		&  	73  		& 	58.2  \\
   katz ,  B = 0.1 	            				& 66.1 		  &   51  	& 	 50 \\
   katz , B= 0.05 	           				& 50.7    	&   51    	&  50  \\
   Topological combined  ALL 		& 87.5       		& 	93   	& 		92 \\
   Topological combined (No PR)  &    69.2 	&   	88      &    89.1 \\ 
   Topological combined (No katz)  							& 86.4.2  & 	89.6            &    89.6  \\ 
   
   katz- matrix , B =0.5 							&   52.0 		&    55  				&   54\\
   katz- matrix , B =0.25 							& 53.0 				&  	54.8  				&  53 \\
   katz- matrix ,  B = 0.1 	            				& 60			    &   54  					& 	 55 \\
   katz- matrix , B= 0.05 	           				& 68     			&   57      		 		&  58  \\   
   Topological combined (No pageRank)  & 69 & 	88           &    87  \\ 
    Topological combined  ALL 		& 87      		& 	93   					& 		92 \\
   
   \midrule
   NMF																					& 52.0    & 54.0 &                53.5 \\
   NMF + Topological combined											& 87  		&  91           &   91 \\
   \midrule
   Motif Combined							 									& 79.6     & 96.0        &   96.5 \\
   \bottomrule
\end{tabular}
\end{table*}


%%%%%%modified comparsion tabl
%% katz= (number of paths of length)^l * B+ ..
%%%%%%modified comparison table
\begin{table*}[tbp]
  \centering
  \caption{New values Accuracy of the RF classifier (\%) when using combined Motif features (\inse) vs baseline features (topological and NMF).}
  \label{tab:comparison2}
  \begin{tabular}{l r r r}
   \toprule
   \textbf{Feature} &	\textbf{Amazon} &	\textbf{CondMat} &	\hspace{1em}\textbf{AstroPh} \\
   \midrule
   Jaccard Coefficient			& 61.7 &81.1&   85.2 \\
   Adamic/Adar						& 61.5 & 74.7    & 75 \\
   Preferential Attachment	& 55.0 & 61. 2  & 64.2 \\
   Common Neighbors			& 64.6 & 78.6    & 81.2 \\
   rooted page rank 				& 66.9 &  64.2   & 63.7\\ 
   katz 0.5 							& 93 &    88  &  85.7 \\
   katz 0.1 							& 95 & 88.7    &  80.7 \\
   katz 0.25 							& 89 &  87.3 &  84.5 \\
   katz 0.05 							& 96 & 90 & 83.0 \\
   Topological combined		& 95.0 & 96.2   & 96.6 \\
   \midrule
   NMF											& 52.0 & 54.0 & 53.5 \\
   NMF + Topological combined	& 96.0 & 96 &  96.6 \\
   \midrule
   Motif Combined							& 79.6 & 96.0 & 96.5 \\
   \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[tbp]
  \centering
  \caption{Accuracy of the RF classifier (\%) when using combined Motif features (\inse) vs baseline features (topological and NMF).}
  \label{tab:comparison}
  \begin{tabular}{l r r r}
   \toprule
   \textbf{Feature} &	\textbf{Amazon} &	\textbf{CondMat} &	\hspace{1em}\textbf{AstroPh} \\
   \midrule
   Jaccard Coefficient		& 61.7 & 75.4 & 74.6 \\
   Adamic/Adar			& 61.5 & 74.7 & 74.9 \\
   Preferential Attachment	& 55.0 & 75.7 & 73.7 \\
   Common Neighbors	& 64.6 & 74.8 & 75.4 \\
   Topological combined	& 66.0 & 87.4 & 86.7 \\
   \midrule
   NMF				& 52.0 & 66.0 & 57.0 \\
   NMF + Topological combined	& 66.0 & 87.0 & 84.0 \\
   \midrule
   Motif Combined		& 79.6 & 96.0 & 96.5 \\
   \bottomrule
\end{tabular}
\end{table*}

%%% BASELINES
\subsection{Comparison with Baselines}
Table~\ref{tab:comparison} reports the accuracy of a Random Forest classifier trained on the different baseline features.
For comparison, we use the Combined motif features extracted via \inse (last row).
The traditional topological features hover around $65$--$75\%$ accuracy across the three datasets.
When combining all the features in a single large vector, the baselines can get up to $66\%$ on Amazon, and $\approx 87\%$ on the other two datasets.

The motif features achieve much higher accuracy: $\approx 80\%$ on Amazon and $\approx 96\%$ on the other two datasets.
That is $9$ to $14$ accuracy percentage points better, which is quite significant, especially given that features extracted via graph embeddings and deep learning reportedly struggle to beat the traditional topological features~\cite{tsitsulin2018verse}.

Interestingly, the NMF approach is not competitive.
The accuracy achieved is up more than $30$ percentage points lower.
We hypothesize that the method requires more parameter optimization (e.g., tuning the number of factors used and the regularization parameters).
In any case, the gap between NMF and straightforward topological features is quite large when used out of the box, which is quite disappointing.
Moreover, adding the NMF features to the topological ones does not improve the accuracy of the classifier.

\spara{Feature importance.}
We analyze the motif features that are most predictive for the classification task.
Figure~\ref{fig:feature-importance} shows the relative importance as inferred by the Random Forest.
In most cases the distribution is quite skewed, with a few features constituting the backbone of the predictive model.
Interestingly, the most predictive feature is always a 5-motif one, which is another indication of the predictive power of deeper structural features.
However, the most important feature changes from dataset to dataset, and might be domain specific.

We trained the RF classifier with just the top-10 features by importance for each dataset, and the accuracy obtained is almost identical to the full model.
This result indicates that feature selection could be used to identify a few important motifs in a dataset, and extract only those, which would reduce the computational burden of counting all the motifs.

Overall, these results prove the predictive power of higher-order motif-based features for link formation.
The rest of the experimental section is devoted to two more questions related to motif feature extraction and negative edge sampling.
First, we shed some insight about why \inse performs better than \rmve.
Second, we show the importance of choosing the right negative examples, an important factor which has been overlooked in the literature.


\begin{figure}
\centering
\subfloat[Amazon]
{\includegraphics[width=0.85\columnwidth]{images/AmazonGImp.pdf}}  \\
\subfloat[CondMat]
{\includegraphics[width=0.85\columnwidth]{images/comImpg.pdf}} \\
\subfloat[AstroPh] 
{\includegraphics[width=0.85\columnwidth]{images/ImpArvix.pdf}} \\
\caption{Feature Importance} 
\label{fig:feature-importance} 
%\todo[inline]{Can you left-align the labels on the y axis?}
\end{figure} 

%three bar charts for each dataset 
%keep the amazon table for remove real edges 
% area under cave for each dataset in one table
% table for false positive rate
%other methods
% classification 
% distribution of motif , distance
% dataset   Emo , LK  
%1           I R   I R 
%2
%3

\begin{table}[tbp]
  \caption{Distances}
  \centering
  \label{tab:distribution}
  \begin{tabular}{l rrrr}
   \toprule
   \textbf{Graph} &  \multicolumn{2}{c}{\textbf{Earth Mover's Distance }}   &  \multicolumn{2}{c}{\textbf{KL Divergence}}  \\
   \cmidrule(lr){2-3}    \cmidrule(lr){4-5}
    &  \multicolumn{1}{c}{\textbf{\rmve}}  &  \multicolumn{1}{c}{\textbf{\inse}}  &  \multicolumn{1}{c}{\textbf{\rmve}}   &  \multicolumn{1}{c}{\textbf{\inse}}   \\    
    \midrule 
    Amazon	& \num{0.118960}	& \num{0.010530}	& \num{0.007129}	& \num{0.000668} \\
    CondMat	& \num{ 1.106199}	& \num{0.160761}	& \num{0.533413}	& \num{0.011669} \\
    AstroPh		& \num{0.049685}	& \num{0.528753}	& \num{0.000539} 	& \num{0.066089} \\
    \bottomrule
\end{tabular}
\end{table}

\subsection{Motifs Distribution: \rmve vs \inse}
\label{sec:distribution}
Let us now look at the reason why \inse outperforms \rmve for feature extraction.
Consider that both feature extraction methods change the original motifs of the graph, as they alter the graph structure during feature extraction.
One hypothesis is that the method which alters the structure the least is better, as the motif patters it learns are also the closest to the ones found in the original graph.
To test this hypothesis, we compute the motif distribution in the original graph, and in the modified graphs resulting from the modifications done by \rmve and \inse (i.e., with a fraction of edges removed or added).
We compute the motif distribution for $k=3,4$ for the whole graph, and compute the distance between the original distribution and the distribution obtained by \rmve and \inse, respectively.
We use two different distance functions to perform the comparison: earth mover's distance %(EMD) 
and Kullback--Leibler divergence. %(KLD).
Table~\ref{tab:distribution} reports the results.
If our hypothesis is correct, then \inse should have a smaller distance than \rmve.
This is indeed the case for two out of three graphs, for both distance function.
However, AstroPh behaves differently.
Therefore, we cannot draw any definitive conclusion with confidence, and further study is necessary to understand the difference between these two  motif feature extraction methods.


\subsection{Effect of Distance Between Negative Edges}
In this experiment we explore the effect of distance between node pairs which constitute the negative examples for the classifier.
For each graph, we create different classification datasets by varying the composition of the negative class:
from containing only negative edges at distance 3 to containing only negative edges at distance 2.
We use the fraction of negative edges of the sub-class at distance 2 as the independent variable in the plots (the rest of the edges are at distance 3).
We keep the total number of the examples fixed to maintain the balance between positive and negative classes.

Figure~\ref{fig:acc-2to3} shows the classification accuracy for each setting.
For both Amazon and ContMat, the edges at distance 2 result harder to classify correctly, which produces a significant decline in the accuracy as we increase the fraction of edges at distance 2.
Conversely, the accuracy on AstroPh does not seem affected.
The same pattern can be seen in Figure~\ref{fig:fpr-2to3}, which reports the false positive rate.
The figure explains the cause of the decrease in accuracy: as we decrease the average distance of the negative examples, the classifier produces more false positives.
The higher the fraction of negative examples at distance two, the higher the rate of misclassification for the negative class.
Again, AstroPh is the exception in our experiments.

We conclude that classification accuracy can be affected by the choice of the negative examples, and that the distance of negative samples should be carefully controlled.
In general, negative examples with smaller distances are harder to classify correctly, as they are more likely to be false positive.
However, the effect remains domain-specific.



\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{images/Fake2Accy.pdf}
\caption{Classification accuracy as a function of the fraction of negative examples at distance 2 (vs distance 3).}
\label{fig:acc-2to3}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{images/Fake2FP.pdf}
\caption{False positive rate as a function of the fraction of negative examples at distance 2 (vs distance 3).}
\label{fig:fpr-2to3}
\end{figure}

\subsection{Motifs Extraction- Time Experiment}

In this experiment, we analysis the time required to extract motifs of size (5) from real and fake edges in Amazon graph. We compute the time in seconds for different number of sample edges (See Figure~\ref{fig:time} ). The results show that the time required for 2000, 20000, 40000 edges is around 4, 6 and 11 hours respectivly. 
\begin{figure}
\centering
\includegraphics[width=0.85\columnwidth]{images/Time.pdf}
\caption{Time required for extracting motifs (m5) for different samples - Amazon Graph }
\label{fig:time}
\end{figure}



==> related2.tex <==
% !TEX root =  vldb_main.tex
\subsection{Literature review} 

The representation of complex real-world relations as graphs has made it possible to systematically investigate the topology and the interaction between the nodes  of these graphs using well-understood graph-theoretical concepts that can be used to predict the structural and dynamical properties of the underlying concepts.

Global measures of graph topology such as the degree distribution %(the degree of a node is the number of edges it participates in) 
and the clustering coefficient  have been thoroughly reviewed in different contexts like cellular networks and proteomics.  
The analysis of the minimum spanning tree was explored as a  suitable method for the comparison of brain networks \cite{tewarie2015minimum}. 
%(the number of edges connecting the neighbours of the node divided by the maximum number of such edges) have recently been thoroughly reviewed in the context of cellular networks [8**] and in proteomics [9].
Methods in path analysis like shortest path algorithms have been well-studied in the domain of road and routing problems \cite{zhan1998shortest}.

More sophisticated techniques like subgraph patterns in the graph (Motifs) have been also explored for different applications . Motifs are patterns of connectivity that occur significantly more frequently in the given graph than expected by chance alone \cite{vazquez2004topological}.

Graph motifs also have numerous other applications: they have been used to classify graphs into “superfamilies” \cite{schneider1991dominant}, they have been used in combination with machine learning techniques to determine the most appropriate network model for a given real-world network \cite{soutoglou2002coordination}. 4-cliques (close motifs of 4 vertexes) reveal community structure in word association and protein-protein interaction graphs \cite{palla2005uncovering}.

In social media analysis studies \cite{juszczyszyn2008local} \cite{juszczyszyn2011link} \cite{ugander2013subgraph}, graph motif detection and numeration problems were addressed  to detect subgraphs of graph and their numeration in order to identify graph properties statistically.

Significance of motifs is typically assessed statistically by comparing the distribution of subgraphs in an observed graph with that found in  randomized graphs that destroy the structure of the graph while preserving the number of nodes, edges and their degree distribution  \cite{vazquez2004topological}.

One of the important reasons why graphs in the real world have a more motif structure than the random version of the graph is that they are constrained by particular types of growth rules which in turn depend on the specific nature of the graph.

Therefore, the present or abundance of recurring sub graphs  or motifs in complex graphs carry significant information about overall organization of the graph \cite{vazquez2004topological}. 
Consequently,  it can help reveal the connections among superficially unrelated biological or social networks  \cite{vazquez2004topological}.

In this research, we evaluate the predication of a link existence between two nodes using this structural unit of graphs as features.

Prior work on link prediction can generally be classified into three categories: similarity measure method, matrix factorization based approach, and probabilistic graphical model method. 

Similarity measure method in link prediction is performed by computing the similarity between a pair of nodes. The higher the similarity between the pair of nodes, the greater the possibility  of a link existing between the node pair in future.
 
There are a variety of  similarity parameters that can be based on application-dependent node attributes or on graph topology.

Similarity based graph topology  parameters  in link prediction can be roughly classified into local, global, and quasi-local approaches.

Global similarity approach  uses global structure information in the graph to measure the similarity of nodes.  Katz index for instance uses the number of paths between two nodes to derive the similarity between them while other methods like Hitting Time, Commute Time, and rooted PageRank use random walks on the graph to derive the similarity of two nodes. Most of global similarity indices often provide  better predictions than local indices but the computation complexity is high especially in large graphs.

Local similarity methods drive the similarity from the direct neighborhood of the involved the nodes, just like Common Neighbors (CN), Jaccard coefficient, Adamic-Adar and Preferential Attachment.

Newman \cite{newman2001clustering} et al. compute the similarity index based on the number of adjacent nodes of the two nodes. the researchers found  that if the two nodes have more identical adjacent nodes, the two nodes will be more likely to generate links.  Jaccard coefficient proposed by Liben-Nowell et al. in \cite{liben2007link} to compute similarity of node pairs by the probability of a neighbor set.  Adamic et al. \cite{adamic2003friends} proposed the Adamic-Adar coefficient, which is a common neighbor  with a a slight modification.
Compared with global index, Local similarity index is fast to compute and scale well in large graphs as their computation depends only on the direct neighborhood of the potential nodes.  However,  they don't have good  accuracy in different kinds of graphs.
The quasi-local structures of graph, which makes compromise between performance and complexity, such as Local Path (LP) or Local Random Walks. LP algorithm considers only two nodes with a path length of 2 or 3, and discarding the longer path.  
This type of similarity measures  capture important patterns or features  between potential nodes without exploring the whole  structure of graph.

Aghabozorgi et al. \cite{aghabozorgi2018new} proposed a triad similarity measure for link prediction between a pair of nodes. The method depends on finding  multiple triple network graphics that the two nodes and their public neighbors belong to. The two nodes completely interact if two nodes and one of their common neighbors form this pattern. The triad similarity measure they proposed is to weight the isomorphism of the node pairs. 

The experiment in \cite{aghabozorgi2018new} shows that the triad similarity measure can obviously improve the accuracy in the link prediction task.  In this paper, we explore this type of similarity and we propose the usage of more complex patterns that contain a pair of nodes to study the existence of a link between them.
%More and more results about similarity measure method have been presented in recent years. 

% In this paper, we demonstrate that this type of similarity can also improve the prediction accuracy. 

Another kind of approachs is to make use of attribute information for link prediction. Examples of node attributes that can be used in unsupervised methods include user profiles in social networks~\cite{wang2015link}, and attributes of publication records in academic co-authorship graphs, such as the topics a researcher works on~\cite{chuan2017link} or the conferences submit to~\cite{liang2017link}. Using node attributes can achieve a high degree of accuracy for link prediction, but it is domain- and application-specific and cannot be generalized.

 Similarity parameters are employed in link prediction using supervised or unsupversied methods. In unsupervised methods, a similarity measure is chosen and used to rank node pairs in the graph, with a higher rank indicating a higher likelihood of a link existing between the node pair~\cite{lu2010link, folino2012link}. For a more detailed survey of unsupervised link prediction methods see the works by~\cite{getoor2005link} and~\cite{lichtenwalter2010new}.
 Different studies indicate that unsupervised methods  are fundamentally unable to cope with dynamics, imbalanced, and other properties in the graphs ~\cite{al2006link}, ~\cite{lichtenwalter2010new}.

Link prediction have been also examined  through unsupervised graph representation and feature learning methods based on node similarity metrics calculated for neighboring nodes. 

Feature Learning methods such as matrix factorization method or neural network based methods are well-known graph feature learning techniques that depend on  the examination of graph topology and structural features to calculate score functions based on pairwise similarity metrics. Common neighbors, preferential attachment, Jaccard, Katz and Adamic Adar are some of the widely used similarity metrics which measure the likelihoods of edge existence in graphs
 
Matrix factorization based approaches, firstly model the graph as a N $X$N matrix in which N represents the number of nodes, and then predict  link by using matrix decomposition of graph theory. Non-negative matrix factorization (NMF) was used to solve link prediction problem.
For example, ~\cite{menon2011link} consider link prediction as a matrix completion problem and solves it using an NMF method. The basic idea is to let the model learn latent features from the topological structure of a partially observed graph, and then use the model to predict whether an edge exist for between unobserved node pairs. This approach is shown to outperform other unsupervised methods such as  Adamic/Adar, preferential attachment, and the Katz measure.  NMF performs best when combining the latent features with features based on node attributes.
In this research, we use only topological features, so we compare our method to NMF using the latent (topological) features, and show that our method significantly outperforms NMF.

Graph Convolutional Networks (GCNs) ~\cite{kipf2016semi} have recently emerged as a powerful tool for representation learning on graphs. GCNs have also been successfully applied for link prediction on normal graphs ~\cite{DBLP:conf/nips/ZhangC18}, ~\cite{schlichtkrull2018modeling}.
 However, the task of link prediction can also be overcome by the use of supervised machine learning algorithms when uses powerful node's features.
 
In supervised method, link prediction problem is usually formalized as a binary classification problem: the target attribute is a class label indicating the existence or absence of a link between a node pair. The predictor attributes are metrics computed from the graph structure or node features, describing the given pair. 

%Supervised Link prediction method is  considered a simple binary classification problem: for any  two potential nodes, predict whether a link exists or not. 
 A key challenge for supervised link prediction is choosing an effective feature set for this task. 
 One types of approaches is to make this prediction  based on topological features of the graph. Liben-Nowell and Kleinberg ~\cite{liben2007link} present a survey of different  predictors based on different graph features.  In a more recent survey ~\cite{gao2015link}, researchers explored different similarity measures.

This approach was first introduced by~\cite{liben2007link}, where graph topological features are used in a study of co-authorship networks. The supervised approach is also used in several later works~\cite{sa2010supervised, leskovec2010predicting, al2006link}. %doppa2009chance 
For a more detailed survey of supervised link prediction methods see~\cite{al2006link}. 

Our proposed  prediction method intend to improve neighborhood-based measures through looking into local structures among nodes (motifs). Therefore, the proposed model is compared with some baseline similarity measures, including: Common Neighbors; Jaccard’s Coefficient; Adamic Adar; Preferential Attachment.  

 Applying supervised model for link prediction requires preparing a training dataset for model learning and a testing dataset for evaluating its performance. In graph context, the features between two nodes  are used for observing connection between them. To ensure that the model will not over-fit to specific set of samples, a set of nodes and existing connection between them must be hidden from the model. One approach to achieve this is to study the graph in different time frames. For instance, edges present in the graph between two time frames used as a training dataset while edges present in the graph  in the later successive time interval form the testing dataset and the aim is to be predicted by the model.  This approach is widely adopted by several studies ~\cite{liben2007link}. 
% As graph grows through the addition of nodes as well as edges, it is not sensible to seek predictions for edges whose endpoints are not present in the training dataset. The edges chosen between time intervals usually belong to the same predefined node set. Thus, the study then evaluate how accurately the new edges between elements of predefined set can be predicted by the model. 
 Proposing a set of non-existing  edges between current endpoints in the graph to form the negative edge list is another method. In the friendship link prediction problem in this work  ~\cite{song2009scalable}, researchers constructed the positive set as the set of user pairs that were not friends in the first snapshot, but become friends in the second snapshot. The negative set consists of user pairs that are friends in neither snapshots

Different graphical models such as  Bayesian Network and Markov Random Field were used in solving link prediction problem.
Luna et al.~\cite{luna2013link}  proposed a link prediction algorithm that combines the probability theory with ontology information and graph-based information to enhance the unavoidable uncertainty in field analysis and tasks. It investigates the scalability of the method through a combination of graph-based features and semantic suppositions. Bhawsar et al. ~\cite{bhawsar2016performance}  proposed two new methods of link prediction based on Markov Random Field and Fuzzy Soft Set. The methods improved the efficiency of similarity measures based on Jaccard, Common Neighbor.
Mart\' inez et al. ~\cite{martinez2017probabilistic} proposed a local link prediction based on the assumption that links that are not discovered in real complex networks may not exist or exist but hide from us. The technique depends on  the presence and absence of uncertainty  to estimate the probability of each possible non-observed link based on observed topological and semantic features. In our research, we tackle improving the accuracy based only on the topological features,  therefore we compare against prior measures that depend on the topological features only regardless of the method or method used.
